VEIL: How Visual Encoding Hijacking Induces Bias In Vision Models

Rendering time series as chart images for CNN-based classification has become increasingly common in time-series classification (TSC). However, it remains unclear whether models learn underlying temporal patterns or rely on encoding-specific visual cues introduced by chart design. We present VEIL: a systematic study examining how chart encodings influence learned representations through complementary analyses of similarity, transferability, and attribution. Attention-guided training appears to mitigate this effect when encoding sensitivity is consistently identified across diagnostics, but provides limited or negative benefit when such signals are absent. These findings position VEIL within the broader question of how machines perceive visualizations -- extending graphical perception from human readers to vision models -- and show that visualization design choices shape learned representations in ways that warrant treating chart-based TSC as a representation and measurement problem rather than a simple modeling decision.

==> acknowledgments.tex <==
\section{Acknowldgements}
This work was supported in part by the U.S. National Science Foundation under Grant No. IIS-2427770.

==> ah_grad.tex <==
\begin{figure}[!t]
  \centering
    \includegraphics[width=\linewidth]{figs_tables/arrowhead_grad.png}
    \subcaption{Grad-CAM overlay}
  \caption{Grad-CAM visualizations for ArrowHead dataset with area chart encoding. (a) Heatmap overlay showing model attention on the original chart image; (b) White mask highlighting the regions most influential for the model's prediction.}
  \label{fig:arrowhead_gradcam}
\end{figure}

==> t1_esi.tex <==
\begin{table}[t!]
  \centering
  \caption{Encoding Sensitivity Index (ESI) for CKA and linear probe across all datasets.}
  \label{tab:esi_summary}
  \begin{tabular}{lcc}
    \hline
    \textbf{Dataset} & \textbf{$\text{ESI}_{\text{CKA}}$} & \textbf{$\text{ESI}_{\text{Probe}}$} \\
    \hline
    Adiac & 0.145 & 0.883 \\
    ArrowHead & 0.282 & 0.681 \\
    Beef & 0.042 & 0.806 \\
    BeetleFly & 0.068 & 0.500 \\
    ChlorineConcentration & 0.275 & 0.637 \\
    Computers & 0.304 & 0.405 \\
    CricketX & 0.131 & 0.438 \\
    CricketY & 0.174 & 0.487 \\
    CricketZ & 0.151 & 0.476 \\
    ECG5000 & 0.016 & 0.184 \\
    GunPoint & 0.238 & 0.497 \\
    Yoga & 0.237 & 0.482 \\
    Strawberry & 0.053 & 0.126 \\
    FordB & 0.464 & 0.489 \\
    Earthquakes & 0.074 & 0.330 \\
    SonyAIBORobotSurface1 & 0.453 & 0.511 \\
    ToeSegmentation1 & 0.355 & 0.509 \\
    ToeSegmentation2 & 0.308 & 0.580 \\
    Wine & 0.065 & 0.508 \\
    WordSynonyms & 0.120 & 0.564 \\
    Ham & 0.215 & 0.496 \\
    Herring & 0.161 & 0.532 \\
    Lightning2 & 0.163 & 0.513 \\
    PhalangesOutlinesCorrect & 0.395 & 0.413 \\
    RefrigerationDevices & 0.490 & 0.586 \\
    SharePriceIncrease & 0.524 & 0.568 \\
    FaceAll & 0.188 & 0.177 \\
    Crop & 0.311 & 0.548 \\
    FacesUCR & 0.121 & 0.489 \\
    Wafer & 0.090 & 0.012 \\
    InsectWingBeat & 0.144 & 0.517 \\
    \hline
  \end{tabular}
\end{table}
